Physics Potentials with the Second Hyper-Kamiokande Detector in Korea

Hyper-Kamiokande consists of two identical water-Cherenkov detectors of total 520~kt with the first one in Japan at 295~km from the J-PARC neutrino beam with 2.5$^{\textrm{o}}$ Off-Axis Angles (OAAs), and the second one possibly in Korea in a later stage. Having the second detector in Korea would benefit almost all areas of neutrino oscillation physics mainly due to longer baselines. There are several candidate sites in Korea with baselines of 1,000$\sim$1,300~km and OAAs of 1$^{\textrm{o}}$$\sim$3$^{\textrm{o}}$. We conducted sensitivity studies on neutrino oscillation physics for a second detector, either in Japan (JD $\times$ 2) or Korea (JD + KD) and compared the results with a single detector in Japan. Leptonic CP violation sensitivity is improved especially when the CP is non-maximally violated. The larger matter effect at Korean candidate sites significantly enhances sensitivities to non-standard interactions of neutrinos and mass ordering determination. Current studies indicate the best sensitivity is obtained at Mt. Bisul (1,088~km baseline, $1.3^\circ$ OAA). Thanks to a larger (1,000~m) overburden than the first detector site, clear improvements to sensitivities for solar and supernova relic neutrino searches are expected.

==> FLAT3.tex <==


%%%%% ==================================================================
%%%%% =====  TODO BELOW HERE ===========================================
%%%%% ==================================================================

%\section{Hyper-K }

%\section{\label{sec:moti} Motivation}
%\pull{


%}



%\pull{As mentioned earlier, the T2HKK experiment consists of the first Hyper-K detector in Kamioka at 295\,km baseline and the second one in Korea at $\sim$1100\,km.  In this document, we assume that the Hyper-K Korean (HKK) detector will be a 258\,kt water Cherenkov detector identical to the Hyper-K detector in Kamioka.}
%---------------------------------------------------------------

%\input{motivation/biProb_t}

%%%=======================================================================================


%In this chapter we present an experimental setup and physics sensitivities of the second Hyper-K detector in Korea using the J-PARC neutrino beam.

%\subsection{J-PARC neutrino beam and Hyper-K detector}

%\subsection




%\clearpage
\begin{figure}[hbt]
\captionsetup{justification=raggedright,singlelinecheck=false}
\centering
\includegraphics[width=1.0\textwidth]{detector/plots/neut-spectra-prob.pdf}
%\end{center}
\caption{Expected J-PARC neutrino (left) and antineutrino (right) spectra and oscillation probabilities at HKK assuming a baseline of 1100 km. Several off-axis angles are considered for comparison. The second oscillation maximum takes place at $\sim$0.7\,GeV at HKK while the first one is at $\sim$2\,GeV.}
\label{neut-spectra-prob}
%\end{center}
\end{figure}


%\input{detector/det_t2hkk_t}

%\subsection
%\input{detector/det_sens_t}
In the following section, some of the quantitative studies are
presented to demonstrate the impact of T2HKK on the Hyper-K project.





==> detector/det_sens_t.tex <==
%%%This file no longer used. Mostly moved to motivation/phys-motiv_t.tex


\graphicspath{{detector/plots}}
\subsection{Improved sensitivity from HKK}

The tiny neutrino mass and the large neutrino mixing compared to quarks indicate that the origin of neutrino mass is from physics beyond the standard model, e.g. the see-saw mechanism. 
Tests of the unitarity of three generation neutrino mixing paradigm would provide an effective tool as demonstrated in quark mixing. Precise determination of the mixing parameters also 
constraints physics beyond the standard model, such as Grand Unification Theory (GUT). For example, precision measurement of CP violation phase $\delta_{CP}$ could distinguish different 
types of flavor symmetries in GUT as shown in Fig.~\ref{fig:GUT-CP}. 

\begin {figure}[htbp]
\captionsetup{justification=raggedright,singlelinecheck=false}
  \begin{center}
\includegraphics[width=0.8\textwidth]{detector/plots/FigcosdeltaNO_fut.pdf}
    \caption{The likelihood function versus $\cos{\delta_{CP}}$ for normal ordering neutrino mass spectrum for different types of flavor symmetries assuming the prospective 1$\sigma$ 
uncertainties in the determination of the neutrino mixing angles~\cite{Petkov2015}.}
    \label{fig:GUT-CP}
  \end{center}
\end {figure}

The complementary information from the second detector in Korea (HKK) at different baseline length could extend the sensitivity of the overall Hyper-K significantly. 
Having both HK and HKK, the J-PARC neutrino beam will provide a compelling measurement to establish CP violation measurement and improve its study of physics beyond the PMNS paradigm. 
Due to a factor of three enhancement of CP violation effect at the second oscillation maximum, the impact of systematic uncertainties is reduced accordingly in T2HKK. 
Systematic uncertainty already has significant impact on the CP sensitivity of T2K-II and it is the main limitation at T2HK. The reduction of impact from systematic uncertainty 
would be very important in establishing the CP violation in the neutrino oscillation. The T2HKK configuration would cover first and second oscillation maxima without serious pion production 
backgrounds at $E_\nu < 1$~GeV. The two different baseline oscillation measurement allows breaking the degeneracy of oscillation parameters and constrains the physics beyond PMNS paradigm. 
Matter effect creates a fake CP violation effect causing difference in $\nu$ and $\bar\nu$ oscillations. The higher energy spectrum of HKK near the first oscillation maximum, 
is in particular sensitive to the matter effect and expected to resolve the mass hierarchy better than 5$\sigma$ level. Other degeneracies of $\delta_{CP}$ and $\theta_{23}$ octant 
or $\Delta m_{31}^2$ can also be constrained. Non-standard neutrino interaction can cause additional matter effect and a new physics beyond PMNS may cause distortion in oscillation pattern. 
Both of these effects can be tested by the two baseline T2HKK data.

In the following section, some of the quantitative studies are presented to demonstrate the impact of T2HKK on the Hyper-K project.


